Operators' cognitive performance under extreme hot-humid exposure and its physiological-psychological mechanism based on ECG, fNIRS, and Eye Tracking

Operators' cognitive functions are impaired significantly under extreme heat stress, potentially resulting in more severe secondary disasters. This research investigated the impact of elevated temperature and humidity (25 60%RH, 30 70%RH, 35 80%RH, 40 90%RH) on the cognitive functions and performance of operators. Meanwhile, we explored the psychological-physiological mechanism underlying the change in performance by electrocardiogram (ECG), functional near-infrared spectroscopy (fNIRS), and eye tracking physiologically. Psychological aspects such as situation awareness, workload, and working memory were assessed. Eventually, we verified and extended the maximal adaptability model to the extreme condition. Unexpectedly, a temporary improvement in simple reaction tasks but rapid impairment in advanced cognitive functions (i.e. situation awareness, communication, working memory) was obtained above 35 WBGT. The best performance in a suitable environment was due to more effective activation in the prefrontal cortex (PFC). With temperature increasing, more mistakes occurred and comprehension was impaired due to drowsiness and lower arousal levels, according to evidence of compensatory effect in fNIRS. In the extreme environment, the enhanced PFC cooperation with higher functional connectivity resulted in a temporary improvement, while depressed activation in PFC, heavy physical load, and poor regulation of the cardiovascular system restricted it. Our results provide a detailed study of the process of operators' performance and cognitive functions when encountering increasing heat stress, as well as its underlying mechanisms from a neuroergonomics perspective. This can contribute to a better understanding of the interaction between operators' performance and workplace conditions, and help to achieve a more reliable human-centered production system in the promising era of Industry 5.0.

==> files/body.tex <==
% ----------------------------- %
% Author Guidelines
% ----------------------------- %
\section{General Guidelines}

\noindent Please read these instructions carefully.   The objective of this template is to enable you in an easy way to style your article attractively in a style similar to that of the typeset journal. It should be emphasized, however, that the final appearance of your paper in print and in electronic media may likely vary to some extent from the presentation achieved in this template.


% ----------------------------- %
% Heading Levels
% ----------------------------- %
\subsection{Level Headings: Subsections}
\noindent You will usually want to divide your article into (numbered) sections and subsections (perhaps even subsubsections).  Use to help organize your document as appropriate.


% ----------------------------- %
% Paragraphs
% ----------------------------- %
\subsection{Paragraphs}
\noindent Paragraphs are \textbf{not} indented and a line break is included between paragraphs.  The first paragraph in a section or subsection will automatically  not  have an indentation.  Use \verb!\noindent! as needed.  


% ----------------------------- %
% Hyperlinks
% ----------------------------- %
\subsection{Hyperlinks / URLs} 
Include hyperlinks using  URL \url{http://www.google.com}.  


% ----------------------------- %
% Mathematics
% ----------------------------- %
\section{Mathematics}\label{sec:lu}
Here is some mathematics.  For $A \in M_n$, the factorization $A = LU$, where $L$ is unit lower triangular and $U$ is upper triangular,  is called the \textit{LU decomposition}, or \textit{LU factorization}.  We can use such a factorization, when it exists, to solve the system $A {\bf x} = {\bf b}$ by first solving for the vector $\bf{y}$ in $L {\bf y} = {\bf b}$ 
and then solving 
$
U {\bf x} = {\bf y}
$. 
However, not every $n \times n$ matrix $A$ has an LU decomposition.  The following theorem provides conditions for the existence and uniqueness of an LU decomposition of a $n \times n$ matrix.  A proof can be found in \citet[p. 160]{johnson1985matrix}.  An equation is given by \cite{strang1993introduction}, 

\begin{equation}\label{eqn:quad}
x = \frac{-b \pm \sqrt{b^2 - 4ac}}{2a}
\end{equation}
  
%: EXAMPLE 1
\begin{example}\normalfont
The $3 \times 3$ matrix  
$A =  \begin{bmatrix}
1 & 5 & 1\\
1 & 4 & 2\\
4 & 10 & 2\\
\end{bmatrix}
$
has all non-zero principle minors, $A_1, A_2$ and $A_3$.  Therefore,  there is a unique LU factorization with both $L$ and $U$ nonsingular given by 
\end{example}
\[
\begin{bmatrix}
1 & 5 & 1\\
1 & 4 & 2\\
4 & 10 & 2\\
\end{bmatrix}
=
\begin{bmatrix}
1 & 0 & 0\\
1 & 1 & 0\\
4 & 10 & 1\\
\end{bmatrix}
\begin{bmatrix}
1 & 5 & 1\\
0 & -1 & 1\\
0 & 0 & 12\\
\end{bmatrix}.
\]



% ----------------------------- %
% Math: Theorems/Defs
% ----------------------------- %
\section{Definition, Theorem, Corollary}


\begin{definition}
Definitions are if and only if statements.  
\end{definition}

\begin{verbatim}
\begin{definition}
Definitions are if and only if statements.  
\end{definition}
\end{verbatim}

%: THEOREM: Infinite LU Factorizations
\begin{theorem}[Matrices with Infinitely Many LU Factorizations]
{For $A \in M_n$, if two or more of any first $(n-1)$ columns are linearly dependent or any of the first $(n-1)$ columns are 0, then $A$ has infinitely many LU factorizations.}
\end{theorem}

%: proof
\begin{proof} We will prove only for the the case when $A \in M_3$. \\
 \begin{align} 
&dm + r = e  \Rightarrow r = e-dm \label{eqn:1}\\
&dn + rp = f \Rightarrow p=\frac{f-dn}{r} \label{eqn:2}\\
&gm + s = h \Rightarrow s = h - gm \label{eqn:3}\\
&gn + sp + t = i \Rightarrow t  = i-sp-gn \label{eqn:4}
\end{align}
 
\end{proof} % end proof
 

% Corollary
\begin{corollary}
If $x$, then $y$.
\end{corollary}



% ----------------------------- %
% Examples
% ----------------------------- %
\section{Examples}\label{ex:x1}
Here is an example of an example.


\begin{example}
Let  $\{1,2,3\}$ and $\{2,1,3\}$ be two lists of integers.  Then, to check if the two lists are equal we would have,   
	\begin{center}
		\texttt{ \{1,2,3\} == \{2,1,3\} }.
	\end{center}\label{ex:equallists}
\end{example}


\begin{verbatim}
\begin{example}
Let  $\{1,2,3\}$ and $\{2,1,3\}$ be two lists of integers.  Then, to check if the two lists are equal we would have,   
	\begin{center}
		\texttt{ \{1,2,3\} == \{2,1,3\} }.
	\end{center}\label{ex:equallists}
\end{example}
\end{verbatim}



% ----------------------------- %
% Lists
% ----------------------------- %
 \section{Lists}
 NAGJ uses the \verb|outline| package.   
  
 % Enumeration
 \subsection{Enumerated List}
 The following code produces an enumerated list.  The enumerated list numbers each list item with Arabic numerals.
 
% Outline
\begin{verbatim}
\begin{outline}[enumerate]
     \1 First Level
          \2 Second level
               \3 Third level
\end{outline}
 \end{verbatim}
 
 % Outline
 \begin{outline}[enumerate]
 	\1 First Level
		\2 Second level
			\3 Third level
\end{outline}
 

 % Itemize
 \subsection{Itemized List}
 The following code produces an itemized list.
 
% Verbatim Outline
\begin{verbatim}
\begin{outline}
     \1 First item
          \2 Second level item
               \3 Third level sub-item
\end{outline}
 \end{verbatim}
 
 % Outline
 \begin{outline}
 	\1 First Level
		\2 Second level
			\3 Third level
\end{outline}



% ----------------------------- %
% Tables and Figures
% ----------------------------- %
\section{Tables and Figures}

A \textbf{caption} that briefly describes the material is required for figures and tables.  Any required information, such as photo credits or data source, may be included in captions. Furthermore, as part of the authorization to use that content, providers of this material may need a specific credit line, which might be placed in the caption (or wherever the provider has requested).  


% ----------------------------- %
% Figures
% ----------------------------- %
 \subsection{Figures}
Figures should be high quality (1200 dpi for line art, 600 dpi for grayscale and 300 dpi for color, at the correct size). The preferred method of including graphics in the \textit{North American GeoGebra Journal} is to export to TiKz.  For exposition on TiKz, see \citep{quinlan2013geogebra}.   
Other acceptable file formats include: EPS, PS, PNG, JPEG, or TIFF.  
  
 \begin{figure}[h!] %  figure placement
    \centering
    \includegraphics[scale=0.5]{figs/venn.pdf} 
    \caption{Provide a short caption description.}
    \label{fig:number}
 \end{figure}
 
 
% ----------------------------- %
% Tables
% ----------------------------- %
\subsection{Tables}
We use the \texttt{booktabs} package.  Tables should present new information rather than duplicating what is in the text. Readers should be able to interpret the table without reference to the text. Please supply editable files.


\begin{table}[ht!]
\begin{center}
\begin{tabular}{lccc} 
	\toprule
	Date & Time  &  Average   & Standard Deviation \\ 
	\midrule
	Jan 1  & 1100	& 4.7		& 0.6		\\
	Jan 2  & 2300	& 16.7	& 2.9		\\
	Jan 3  & 1400	& 11.4	& 3.5		\\
	Jan 4  & 1130	& 8.4		& 2.1		\\
	Jan 5  & 500	& 5.2		& 1.9		\\
	Jan 6  & 1700	& 7.9		& 2.2		\\
	\bottomrule 
\end{tabular} 
\caption{This is a caption to the table}
\label{tab:1} 
\end{center}
\end{table} % end the table



% ----------------------------- %
% Cross Referencing
% ----------------------------- %
\section{Cross Reference}
Figures, tables, and equations should be labeled (\texttt{label}) then referenced using the \texttt{ref}. 


% ----------------------------- %
% Citations
% ----------------------------- %
\section{Citations}
Citations follow APA format.  \citet{johnson1985matrix} shows an example using \verb!\citet{key}!, whereas to include citations parenthetically as in, \citep{johnson1985matrix}, use \verb!\citep{key}!.  You can also include page number of reference such as, \citep[p. 17]{johnson1985matrix}, by using options in the cite command, i.e.,  \verb!\citep[p. 17]{key}!.  Multiple researchers \citep{johnson1985matrix,strang1993introduction} can be cited using one cite command; in particular, with keys separated by commas  \verb!\citep{johnson1985matrix,strang1993introduction}!.



% ----------------------------- %
% GeoGebra Commands
% ----------------------------- %
\section{GeoGebra Command Line}
Commands that could be entered at the GeoGebra command prompt should use the \verb!verbatim! environment and can be centered.
\begin{center}
\verb! J=(6-(16/3-distance(D,K)),y(C)).!
\end{center}
For inline commands such as \texttt{distance(A,B)}, use \verb!\texttt! or \verb!\verb!.   


% ----------------------------- %
% Appendix
% ----------------------------- %
\section*{Appendix}
Appendixes, if needed, appear before the acknowledgment.



% ----------------------------- %
% Acknowledgment
% ----------------------------- %
\section*{Acknowledgment}
The preferred spelling of the word ``acknowledgment" in American English is without an ``e" after the ``g." Use the singular heading even if you have many acknowledgments. Avoid expressions such as ``One of us (S.B.A.) would like to thank ... ." Instead, write ``F. A. Author thanks ... ." In most cases, sponsor and financial support acknowledgments are placed in the unnumbered footnote on the first page, not here.



